Learning Domain-Specialised Representations for Cross-Lingual Biomedical Entity Linking

Injecting external domain-specific knowledge (e.g., UMLS) into pretrained language models (LMs) advances their capability to handle specialised in-domain tasks such as biomedical entity linking (BEL). However, such abundant expert knowledge is available only for a handful of languages (e.g., English). In this work, by proposing a novel cross-lingual biomedical entity linking task (XL-BEL) and establishing a new XL-BEL benchmark spanning 10 typologically diverse languages, we first investigate the ability of standard knowledge-agnostic as well as knowledge-enhanced monolingual and multilingual LMs beyond the standard monolingual English BEL task. The scores indicate large gaps to English performance. We then address the challenge of transferring domain-specific knowledge in resource-rich languages to resource-poor ones. To this end, we propose and evaluate a series of cross-lingual transfer methods for the XL-BEL task, and demonstrate that general-domain bitext helps propagate the available English knowledge to languages with little to no in-domain data. Remarkably, we show that our proposed domain-specific transfer methods yield consistent gains across all target languages, sometimes up to 20 Precision@1 points, without any in-domain knowledge in the target language, and without any in-domain parallel data.

==> history.tex <==
\begin{table}[!h]
\tiny
\setlength{\tabcolsep}{1.0pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.9}
%\vspace{-0.5em}
%\vspace{-0.5em}
\centering
\begin{tabular}{llccccccccccccccccccccccccccccc}
\toprule
  language$\rightarrow$& \multicolumn{2}{c}{en} & $\ $ & \multicolumn{2}{c}{es} & $\ $ & \multicolumn{2}{c}{de} & $\ $ &  \multicolumn{2}{c}{eu} & $\ $ &  \multicolumn{2}{c}{ru} & $\ $ &  \multicolumn{2}{c}{zh} & $\ $ &  \multicolumn{2}{c}{ja} &  $\ $ &  \multicolumn{2}{c}{th}\\
 \cmidrule{2-3}\cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15} \cmidrule{17-18}\cmidrule{20-21}
  model$\downarrow$ &  {\scriptsize @1} &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5  \\
  \midrule
  \textsc{SapBert} \citep{liu2020self} & \textbf{78.7} & \textbf{81.6} && & && 22.7 & 24.7 &&50.8 & 54.1 && 5.8 & 6.0 && 1.9 & 2.2 && 3.0 & 3.2 && 3.1 & 3.4 \\
    \textsc{SapBert}$_{\text{all\_syn}}$ & 78.3 & 80.7 && &&& 30.0 & 34.2 && 58.1 & 62.4 && 9.3 & 11.3 && 6.4 & 8.2 && 6.9 & 8.3 && 3.0 & 3.3\\
     \hdashline
    \textsc{deBert} & & &&  &&&  16.8 & 18.4 \\
  \textsc{deBert}$_{\textsc{nospec}}$ & & &&  &&&  9.5 & 12.1 \\
    \textsc{deBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&  \textbf{35.5} & \textbf{40.0} \\
     \hdashline
 \textsc{zhBert} & &  &&&  && & && & && & && 2.1 & 3.2 \\
\textsc{zhBert}$_{\textsc{nospec}}$ & & && & && & && &  &&&  && 1.5 & 1.9\\
 \textsc{zhBert+SapBert}$_{\text{all\_syn}}$ & & && & &&  &&&  & && & && 18.5 & \textbf{23.8}  \\

 \hdashline
 \textsc{jaBert} & & &&  &&& & && & && & && & && 2.7 & 2.8 \\
\textsc{jaBert}$_{\textsc{nospec}}$ & & && & && & && & && &&&  & && 1.9 & 2.5 &\\
 \textsc{jaBert+SapBert}$_{\text{all\_syn}}$ & & && & && &&&  & && & && & && 21.2 & 25.9 \\
  \midrule
    \textsc{mBert} & 0.8 & 1.7 &&  &&& 0.3 & 0.4 && 0.4 & 0.8 && 0.0 & 0.0 &&  0.0 & 0.0 && 0.0 & 0.1 && 0.0 & 0.0\\
  \textsc{mBert}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} & 35.8  & 49.4 &&  &&& 7.1 & 10.4 && 20.3 & 30.1 && 2.3 & 3.6 && 0.9 & 1.4 && 1.7 & 2.2 && 1.1 & 1.7 \\
   \textsc{mBert+SapBert}$_{\text{en\_syn}}$ & 75.5 & 79.9 &&  &&& 26.0 & 29.6 && 51.0 & 54.5 && 10.1 & 12.6 && 4.1 & 5.7 && 4.7 & 5.9 && 3.1 & 3.5 \\
   \textsc{mBert+SapBert}$_{\text{all\_syn}}$ & 75.0 & 79.7 &&  &&&  33.4 & 37.8 && \textbf{60.6} & \textbf{63.9} && 35.1 & 40.3 && 19.5 & 22.7 && 19.9 & 25.0 && 2.8 & 3.4 \\
     \hdashline  
\textsc{XLMR}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} &  0.2 & 0.4 \\
\textsc{XLMR}$_{\textsc{mean\_pool}}$ & 0.2 & 0.5 \\ 
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$ & 78.1 & 80.9 && &&&  27.6 & 32.0 && 55.9 & 60.8 && 21.8 & 25.9 && 7.9 & 11.3 && 8.3 & 11.3 && 11.5 & 16.2 \\
\textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$ & 78.6 & 81.3 && &&&  29.7 & 36.4 && 56.3 & 61.8 && 29.3 & 33.5 && 16.1 & 20.6 && 22.8 & 27.7 && 20.2 & 26.4 \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$ & 78.2 & 81.0 && 56.4 & 62.7 & & 31.8 & 37.3 && 58.0 & 63.5 && \textbf{35.4} & \textbf{41.2} && \textbf{18.8} & 23.0 && \textbf{24.0} & \textbf{28.1} && \textbf{20.6} & \textbf{27.5}   \\
\hline  
%\small\color{red} Latest results (general-domain parallel data):\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de wt}}$ \textsc{XMLR} & & & &&&  & 13.2 & 18.1\\
  \textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de muse}}$ \textsc{XMLR} & & & & &&&  6.8 & 9.8 \\
 %\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-zh wt}}$ \textsc{XMLR} \\
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th wt}}$ \textsc{XMLR} & &  & && && & &&& & && && && && && 1.4 & 3.7 \\
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th muse}}$ \textsc{XMLR} & & &&&   & && && && && && && && && 0.1 & 0.2 \\


\hdashline
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de wt) & &  &&&  & & 34.6 & 41.4 & && && && && && && &&\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de muse) &  &&& &  && 28.7 & 34.4 && && && && && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de wt+muse) & &&&  &  &  & 30.3 & 36.9 && && && &&  & && &&  \\
 
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh wt) & &  &&&  & && && && && && 15.9 & 23.0 & && && &&\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh muse) & &  &&&  & && && && && & & 12.3 & 16.7 & && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh wt+muse) & &  &&& & && &&& && & &&16.0 & 22.9    \\

 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th wt) & &  &&&  & && && && && && && && && 25.1 & 32.4 \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th muse) & &  &&&  & && && && && && && && && 18.6 & 25.1 \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th wt+muse) & &  &&&  & && && && && && && && && 26.2 & 34.0 \\
 
 \hdashline
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de wt) &  &&&  && & 34.4 & 40.9 & && && && \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de muse) &  &&& && & 32.6 & 36.8 & && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de wt+muse) & &&&  && & 32.0 & 39.4 & && && && \\
 
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh wt) & &  &&&  & && && && & & & & 20.5 & 27.5 && && \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh muse) & &  &&&  & && && && & & & & 16.5 & 21.0 && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh wt+muse) &  &&& &  & && && && & & & & 21.3 & 28.8 && &&   \\

  \textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$(+en-th wt) & &  &&&  & && && && && && && && & & 29.8 & 36.4 &  \\

 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-th muse) & &  &&&  & && && && && && && && & & 26.6 & 32.2 & \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-th wt+muse)& &  &&&  & && && && && && && && & & 29.0 & 36.3 & \\
  \textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$(+en-th ted) & &  &&&  & && && && && && && && & & 21.1 & 27.9 &  \\
 \hdashline
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de wt) & &  &&&  && 35.1 & 42.3 \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de muse) & &   &&&  &&  33.0 & 38.4 && && && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de wt+muse) & &  &&&  && 31.3 & 38.9 && && && && &&   \\
 
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh wt)  & &  &&&  & & & & && && & && 20.6 & 27.3 & & & \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh muse) & &  &&&  & & & & && && & && 19.2 & 25.6 & & &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh wt+muse) & &  &&&  & & & & && && & && 21.1 & 28.2 & & & \\

 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th wt) & &  &&&  & && && && && && && && & & 30.0 & 37.6 &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th muse) & &  &&&  & && && && && && && && & & 25.9 & 32.8 &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th wt+muse)  &&&  & &  & && && && && && && && & & 30.9 & 37.9 &  \\
\bottomrule
\end{tabular}
\caption{Zero-shot results on 1k randomly selected test set. All mentions in the 1k set have different surface forms from their linked titles. Note that for speeding up testing, the target ontology is a subset of UMLS: only the concepts appear in WikiMed are included. Without explicit mentioning, \texttt{[CLS]} is used as the representation. \textbf{Notations}: ``$\leftarrow$'' means knowledge distillation \citep{reimers2020making}; ``(+$\cdot$)'' means further pre-training;``wt'' means Wikipedia title pairs (collected from latest wiki dump); ``muse'' means word translation pairs (\url{https://github.com/facebookresearch/MUSE}); q``ted'' means the TED2020 dataset by \citet{reimers2020making}.}
%\vspace{-1.5em}
\end{table}


% Jan 21, 2021
\begin{table}[!h]
\tiny
\setlength{\tabcolsep}{1.0pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.9}
%\vspace{-0.5em}
%\vspace{-0.5em}
\centering
\begin{tabular}{llccccccccccccccccccccccccccccc}
\toprule
  language$\rightarrow$& \multicolumn{2}{c}{en} & $\ $ & \multicolumn{2}{c}{es} & $\ $ & \multicolumn{2}{c}{de} & $\ $ &  \multicolumn{2}{c}{fi} & $\ $ &  \multicolumn{2}{c}{ru} & $\ $ & 
  \multicolumn{2}{c}{tr} & $\ $ &
  \multicolumn{2}{c}{ko} & $\ $ & \multicolumn{2}{c}{zh} & $\ $ &  \multicolumn{2}{c}{ja} &  $\ $ &  \multicolumn{2}{c}{th}\\
 \cmidrule{2-3}\cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15} \cmidrule{17-18}\cmidrule{20-21}\cmidrule{23-24}\cmidrule{26-27}\cmidrule{29-30}
  model$\downarrow$ &  {\scriptsize @1} &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5  \\
  \midrule
  \textsc{SapBert} \citep{liu2020self} & \textbf{78.7} & \textbf{81.6} && 47.3 & 51.4 && 22.7 & 24.7 && 8.2 & 10.2 && 5.8 & 6.0 && 26.4 & 29.7 && 2.0 & 2.4 && 1.9 & 2.2 && 3.0 & 3.2 && 3.1 & 3.4 \\
    \textsc{SapBert}$_{\text{all\_syn}}$ & 78.3 & 80.7 && 55.6 & 61.3 && 30.0 & 34.2 && 11.8 & 14.8 && 9.3 & 11.3 && &&&  &&&  6.4 & 8.2 && 6.9 & 8.3 && 3.0 & 3.3\\
     \hdashline
    \textsc{esBert} & & && 41.3 & 42.5 && \\
    \textsc{esBert}$_{\textsc{nospec}}$ & & && 42.1 & 44.2 && \\
    \textsc{esBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&   \\
     \hdashline
    \textsc{deBert} & & &&  &&&  16.8 & 18.4 \\ 
  \textsc{deBert}$_{\textsc{nospec}}$ & & &&  &&&  9.5 & 12.1 \\
    \textsc{deBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&  \textbf{35.5} & \textbf{40.0} \\
\hdashline
    \textsc{fiBert} & & &&  &&& && &  4.9 & 5.2 \\
    \textsc{fiBert}$_{\textsc{nospec}}$ & & &&  &&& && & 2.4 & 3.3 \\
    \textsc{fiBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&   \\
\hdashline
    \textsc{ruBert}& & &&  &&& && &  & && 1.1 & 1.6 \\
\textsc{ruBert}$_{\textsc{nospec}}$ & & &&  &&& && &  & && 2.4 & 3.5 \\
    \textsc{ruBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&   \\
\hdashline
    \textsc{trBert} & & &&  &&&  &&  &&&  &&  && 19.5 & 21.8 \\
    \textsc{trBert}$_{\textsc{nospec}}$ & & &&  &&&  &&  &&&  &&  && 24.1 & 25.8\\
    \textsc{trBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&  &&  &&&  &&  && 44.9 & 49.7 \\
\hdashline
    \textsc{koBert} & & &&  &&&  &&  &&&  &&  &&& && 1.1 & 1.6 \\
    \textsc{koBert}$_{\textsc{nospec}}$  & & &&  &&&  &&  &&&  &&  &&& && 0.1 & 0.4 \\
    \textsc{koBert+SapBert}$_{\text{all\_syn}}$ & & &&  &&&   \\
     \hdashline
 \textsc{zhBert} & &  &&&  && & && & && & &&  &&&  &&& 2.1 & 3.2 \\
\textsc{zhBert}$_{\textsc{nospec}}$ & & && & && & && &  &&&  &&  &&&  &&& 1.5 & 1.9\\
 \textsc{zhBert+SapBert}$_{\text{all\_syn}}$ & & && & &&  &&&  & && & &&  &&&  &&& 18.5 & \textbf{23.8}  \\

 \hdashline
 \textsc{jaBert} & & &&  &&& & && & && & && & &&  &&&  &&& 2.7 & 2.8 \\
\textsc{jaBert}$_{\textsc{nospec}}$ & & && & && & && & && &&&  & && &&&  &&&  1.9 & 2.5 &\\
 \textsc{jaBert+SapBert}$_{\text{all\_syn}}$ & & && & && &&&  & && & && & &&  &&&  &&& 21.2 & 25.9 \\
 \hdashline
     \textsc{thBert} & & && && && &&& && &&& &&&&& &&  &&& && 0.4 & 0.4  \\
    \textsc{thBert}$_{\textsc{nospec}}$ & & && && && &&& && &&& &&&&& &&  &&& && 0.5 & 0.5 \\
    \textsc{thBert+SapBert}$_{\text{all\_syn}}$  \\
  \midrule
    \textsc{mBert} & 0.8 & 1.7 &&  0.5 & 0.7 && 0.3 & 0.4 && 0.4 & 0.8 && 0.0 & 0.0 && 0.7 & 1.2 && 0.0 & 0.0 &&  0.0 & 0.0 && 0.0 & 0.1 && 0.0 & 0.0\\
  \textsc{mBert}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} & 35.8  & 49.4 && 15.0 & 24.1 && 7.1 & 10.4 && 1.7 & 2.6 && 2.3 & 3.6 && 10.8 & 15.3 &&  1.3 & 1.7 && 0.9 & 1.4 && 1.7 & 2.2 && 1.1 & 1.7 \\
   \textsc{mBert+SapBert}$_{\text{en\_syn}}$ & 75.5 & 79.9 && 50.6 & 55.8 && 26.0 & 29.6 && 8.7 & 10.7 && 10.1 & 12.6 && 31.0 & 34.4 && 2.7 & 3.2 && 4.1 & 5.7 && 4.7 & 5.9 && 3.1 & 3.5 \\
   \textsc{mBert+SapBert}$_{\text{all\_syn}}$ & 75.0 & 79.7 && 61.4 & 67.0 &&  33.4 & 37.8 && 18.4 & 21.9 && 35.1 & 40.3 && 44.5 & 47.7 && 15.1 & 17.6 && 19.5 & 22.7 && 19.9 & 25.0 && 2.8 & 3.4 \\
     \hdashline  
\textsc{XLMR}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} &  0.2 & 0.4 \\
\textsc{XLMR}$_{\textsc{mean\_pool}}$ & 0.2 & 0.5 \\ 
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$ & 78.1 & 80.9 && 47.9 & 53.5 &&  27.6 & 32.0 && 12.2 & 14.7 && 21.8 & 25.9 && 29.3 & 35.9 && 4.5 & 6.7 && 7.9 & 11.3 && 8.3 & 11.3 && 11.5 & 16.2 \\
\textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$ & 78.6 & 81.3 &&  &  &&  29.7 & 36.4 &&  &  && 29.3 & 33.5 &&  & &&  &&& 16.1 & 20.6 && 22.8 & 27.7 && 20.2 & 26.4 \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$ & 78.2 & 81.0 && 56.4 & 62.7 & & 31.8 & 37.3 && 18.6 & 22.2 && \textbf{35.4} & \textbf{41.2} && 42.8 & 48.9 && 16.7 & 21.4 && \textbf{18.8} & 23.0 && \textbf{24.0} & \textbf{28.1} && \textbf{20.6} & \textbf{27.5}   \\
\hline  
%\small\color{red} Latest results (general-domain parallel data):\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de wt}}$ \textsc{XMLR} & & & &&&  & 13.2 & 18.1\\
  \textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de muse}}$ \textsc{XMLR} & & & & &&&  6.8 & 9.8 \\
 %\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-zh wt}}$ \textsc{XMLR} \\
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th wt}}$ \textsc{XMLR} & &  & && && & &&& & && && && && && &&&  &&&  1.4 & 3.7 \\
\textsc{XMLR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th muse}}$ \textsc{XMLR} & & &&&  &&&   & && && && && && && && &&  &&& 0.1 & 0.2 \\


\hdashline
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de wt) & &  &&&  & & 34.6 & 41.4 & && && && && && && &&\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de muse) &  &&& &  && 28.7 & 34.4 && && && && && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-de wt+muse) & &&&  &  &  & 30.3 & 36.9 && && && &&  & && &&  \\
 
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh wt) & &  &&&  & && && && && && &&&  &&&  15.9 & 23.0 & && && &&\\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh muse) & &  &&&  & && && && && & &  &&&  &&& 12.3 & 16.7 & && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-zh wt+muse) & &  &&& & && &&& && & &&  &&&  &&& 16.0 & 22.9    \\

 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th wt) & & &&&  & && && && && && && && &&  &&&  &&& 25.1 & 32.4 \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th muse) & &  &&&  &&&  & && && && && && && && && &&&  18.6 & 25.1 \\
 \textsc{XMLR+SapBert}$_{\text{en\_syn}}$(+en-th wt+muse) & &  &&&  &&&  & && && && && && && &&  &&& && 26.2 & 34.0 \\
 
 \hdashline
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de wt) &  &&&  && & 34.4 & 40.9 & && && && \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de muse) &  &&& && & 32.6 & 36.8 & && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-de wt+muse) & &&&  && & 32.0 & 39.4 & && && && \\
 
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh wt) & &  &&&  & && && && & & & &  &&&  &&& 20.5 & 27.5 && && \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh muse) & &  &&&  & && && && & & & &  &&& &&& 16.5 & 21.0 && &&  \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-zh wt+muse) &  &&& &  & && && && & & & &  &&&  &&&  21.3 & 28.8 && &&   \\

  \textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$(+en-th wt) & &  &&&  & && && && && && && && & &  &&&  &&& 29.8 & 36.4 &  \\

 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-th muse) & &  &&&  &&&  & && && && && && && && & &  &&&  26.6 & 32.2 & \\
 \textsc{XMLR+SapBert}$_{\text{en-tgt\_syn}}$(+en-th wt+muse)& &  &&&  &&&  & && && && && && && && & &  &&& 29.0 & 36.3 & \\
  \textsc{XMLR+SapBert}$_{\text{all-tgt\_syn}}$(+en-th ted) & &  &&&  &&&  & && && && && && && && & &  &&& 21.1 & 27.9 &  \\
 \hdashline
 

  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-lang wt) & - & - && 57.2 & 63.7  && 35.1 & 42.3 && & && & && & && 22.1 & 27.9 && 20.6 & 27.3 && & && 30.0 & 37.6 \\
    \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-lang muse) & - & - &&  57.9 & 63.9 && 33.0 & 38.4 && 23.0 & 27.3 && 39.8 & 45.9 && 47.2 & 54.5 && 22.1 & 25.7 && 19.2 & 25.6 && 25.2 & 30.2 && 25.9 & 32.8  \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-lang muse+wt) & - & - &&  51.4 & 61.2 && 31.3 & 38.9 && 22.8 & 28.4 && & && & && & && 21.1 & 28.2 && & &&  30.9 & 37.9 \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de wt) & &  &&&  && 35.1 & 42.3 \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de muse) & &   &&&  &&  33.0 & 38.4 && && && && &&  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-de wt+muse) & &  &&&  && 31.3 & 38.9 && && && && &&   \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-fi wt)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\
    \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-fi muse)  & &  &&&  &&&  & & 23.0 & 27.3 & && && & &&  &&& & & & \\
   \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-fi wt+muse)  & &  &&&  &&&  & & 22.8 & 28.4 & && && & &&  &&& & & &\\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ru wt)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\
      \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ru muse)  & &  &&&  &&&  & & & && 39.8 & 45.9 && && & \\
   \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ru wt+muse)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-tr wt)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\
     \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-tr muse)  & &  &&&  &&&  & & & && && & 47.2 & 54.5 & & \\
   \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-tr wt+muse)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\
  \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ko wt)  & &  &&&  &&&  & & & && && & && & 22.1 & 27.9  \\
     \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ko muse)  & &  &&&  &&&  & & & && && & && & 22.1 & 25.7 & \\
\textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ko wt+muse)  & &  &&&  &&&  & & & & && && & &&  &&& & & & \\

 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh wt)  & &  &&&  &&&  & & & & && && & &&  &&& 20.6 & 27.3 & & & \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh muse) & &  &&&  &&&  & & & & && && & &&  &&& 19.2 & 25.6 & & &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-zh wt+muse) & &  &&&  &&&  & & & & && && & &&  &&& 21.1 & 28.2 & & & \\
 
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ja wt) & &  &&&  & && && && && && && && & &  &&&  &&&  &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ja muse) & &  &&&  &&&  & && && && && && && && && 25.2 & 30.2 &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-ja wt+muse)  &&&  &&&  & &  & && && && && && && && & &  &&&  &  \\
 
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th wt) & &  &&&  & && && && && && && && & &  &&&  &&& 30.0 & 37.6 &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th muse) & &  &&&  &&&  & && && && && && && && & &  &&& 25.9 & 32.8 &  \\
 \textsc{XMLR+SapBert}$_{\text{all\_syn}}$(+en-th wt+muse)  &&&  &&&  & &  & && && && && && && && & &  &&& 30.9 & 37.9 &  \\
\bottomrule
\end{tabular}
\caption{Zero-shot results on 1k randomly selected test set. All mentions in the 1k set have different surface forms from their linked titles. Note that for speeding up testing, the target ontology is a subset of UMLS: only the concepts appear in WikiMed are included. Without explicit mentioning, \texttt{[CLS]} is used as the representation. \textbf{Notations}: ``$\leftarrow$'' means knowledge distillation \citep{reimers2020making}; ``(+$\cdot$)'' means further pre-training;``wt'' means Wikipedia title pairs (collected from latest wiki dump); ``muse'' means word translation pairs (\url{https://github.com/facebookresearch/MUSE}); q``ted'' means the TED2020 dataset by \citet{reimers2020making}.}
%\vspace{-1.5em}
\end{table}


% Jan. 29th
\begin{table*}[!h]
\scriptsize
\setlength{\tabcolsep}{1.0pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.9}
%\vspace{-0.5em}
%\vspace{-0.5em}
\centering
\begin{tabular}{llccccccccccccccccccccccccccccccc}
\toprule
  language$\rightarrow$& \multicolumn{2}{c}{en} & $\ $ & \multicolumn{2}{c}{es} & $\ $ & \multicolumn{2}{c}{de} & $\ $ &  \multicolumn{2}{c}{fi} & $\ $ &  \multicolumn{2}{c}{ru} & $\ $ & 
  \multicolumn{2}{c}{tr} & $\ $ &
  \multicolumn{2}{c}{ko} & $\ $ & \multicolumn{2}{c}{zh} & $\ $ &  \multicolumn{2}{c}{ja} &  $\ $ &  \multicolumn{2}{c}{th} &  $\ $ &  \multicolumn{2}{c}{avg}\\
 \cmidrule{2-3}\cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12} \cmidrule{14-15} \cmidrule{17-18}\cmidrule{20-21}\cmidrule{23-24}\cmidrule{26-27}\cmidrule{29-30}\cmidrule{32-33}
  model$\downarrow$ &  {\scriptsize @1} &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5 & &\scriptsize @1 &\scriptsize @5  \\
  \midrule
  \textsc{SapBert} \citep{liu2020self} & \textbf{78.7} & \textbf{81.6} && 47.3 & 51.4 && 22.7 & 24.7 && 8.2 & 10.2 && 5.8 & 6.0 && 26.4 & 29.7 && 2.0 & 2.4 && 1.9 & 2.2 && 3.0 & 3.2 && 3.1 & 3.4 && \\
    \textsc{SapBert}$_{\text{all\_syn}}$ & 78.3 & 80.7 && 55.6 & 61.3 && 30.0 & 34.2 && 11.8 & 14.8 && 9.3 & 11.3 && 35.5 & 39.5 && 2.0 & 2.4 && 6.4 & 8.2 && 6.9 & 8.3 && 3.0 & 3.3\\
     \hdashline
    \{\$LANG\}\textsc{Bert} & - & - && 41.3 & 42.5 && 16.8 & 18.4 && 4.9 & 5.2 && 1.1 & 1.6 && 19.5 & 21.8 && 1.1 & 1.6 && 2.1 & 3.2 && 2.7 & 2.8 && 0.4 & 0.4 \\  
    \{\$LANG\}\textsc{Bert}$_{\textsc{nospec}}$ & - & - && 42.1 & 44.2 && 9.5 & 12.1 && 2.4 & 3.3 && 2.4 & 3.5 && 24.1 & 25.8 && 0.1 & 0.4 && 1.5 & 1.9 && 1.9 & 2.5 && 0.5 & 0.5 \\
    \{\$LANG\}\textsc{Bert+Sap}$_{\text{all\_syn}}$ & - & - && 60.9 & 66.8 && 35.5 & 40.0 && 18.8 & 23.9 &&  36.4 & 42.4 && 44.9 & 49.7 && 13.5 & 16.0 && 18.5 & 23.8 && 21.2 & 25.9 && 0.6 & 0.6 \\
  \midrule
    \textsc{mBert} & 0.8 & 1.7 &&  0.5 & 0.7 && 0.3 & 0.4 && 0.4 & 0.8 && 0.0 & 0.0 && 0.7 & 1.2 && 0.0 & 0.0 &&  0.0 & 0.0 && 0.0 & 0.1 && 0.0 & 0.0\\
  \textsc{mBert}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} & 35.8  & 49.4 && 15.0 & 24.1 && 7.1 & 10.4 && 1.7 & 2.6 && 2.3 & 3.6 && 10.8 & 15.3 &&  1.3 & 1.7 && 0.9 & 1.4 && 1.7 & 2.2 && 1.1 & 1.7 \\
   \textsc{mBert+Sap}$_{\text{en\_syn}}$ & 75.5 & 79.9 && 50.6 & 55.8 && 26.0 & 29.6 && 8.7 & 10.7 && 10.1 & 12.6 && 31.0 & 34.4 && 2.7 & 3.2 && 4.1 & 5.7 && 4.7 & 5.9 && 3.1 & 3.5 \\
   \textsc{mBert+Sap}$_{\text{all\_syn}}$ & 75.0 & 79.7 && \textbf{61.4} & \textbf{67.0} && 33.4 & 37.8 && 18.4 & 21.9 && 35.1 & 40.3 && 44.5 & 47.7 && 15.1 & 17.6 && 19.5 & 22.7 && 19.9 & 25.0 && 2.8 & 3.4 \\
     \hdashline  
\textsc{XLMR}$_{\textsc{nospec}}$ \tiny\citep{vulic-etal-2020-probing} &  0.2 & 0.4 \\
\textsc{XLMR}$_{\textsc{mean\_pool}}$ & 0.2 & 0.5 \\ 
\textsc{XLMR+Sap}$_{\text{en\_syn}}$ & 78.1 & 80.9 && 47.9 & 53.5 &&  27.6 & 32.0 && 12.2 & 14.7 && 21.8 & 25.9 && 29.3 & 35.9 && 4.5 & 6.7 && 7.9 & 11.3 && 8.3 & 11.3 && 11.5 & 16.2 \\
\textsc{XLMR+Sap}$_{\text{es\_syn}}$ & & && 52.9 & 58.8\\
\textsc{XLMR+Sap}$_{\text{en+es\_syn}}$ & & && 55.8 & 62.5\\
\textsc{XLMR+Sap}$_{\text{de\_syn}}$ & & && & && 25.9 & 30.4 &&  \\
\textsc{XLMR+Sap}$_{\text{en+de\_syn}}$  \\
%\textsc{XLMR+Sap}$_{\text{all-es\_syn}}$ & & && \\
\textsc{XLMR+Sap}$_{\text{ru\_syn}}$ & & && && && && && &28.7 & 34.2 \\
\textsc{XLMR+Sap}$_{\text{en+ru\_syn}}$ & & && && && && && & 36.4 & 42.2 \\
%\textsc{XLMR+Sap}$_{\text{all-ru\_syn}}$ & & && \\
\textsc{XLMR+Sap}$_{\text{ko\_syn}}$ & & && && && && && && && && & 2.4 & 2.9 \\
\textsc{XLMR+Sap}$_{\text{en+ko\_syn}}$ & & && && && && && && && && & 15.8 & 19.8\\
%\textsc{XLMR+Sap}$_{\text{all-ko\_syn}}$ & & && \\
\textsc{XLMR+Sap}$_{\text{tgt\_syn\_only}}$ & 77.5 & 80.3 && 55.3 & 61.8 && 31.5 & 36.6 && 18.7 & 23.4 && 34.6 & 40.6 && 40.9 & 45.6 && 16.0 & 21.0 && 14.7 & 19.1 && 14.1 & 18.9 && 19.3 & 25.2 \\
\textsc{XLMR+Sap}$_{\text{en+tgt\_syn}}$ & 77.9 & 80.9 && 55.2 & 61.6 && 32.4 & 37.8 && 17.9 & 21.7 && 35.2 & 41.3 && 40.3 & 46.9 && 16.0 & 20.5 && 17.5 & 22.2 && 14.7 & 18.5 && 17.7 & 23.4 \\
\textsc{XLMR+Sap}$_{\text{all-tgt\_syn}}$ & 78.2 & 80.8 && 53.9 & 60.0 && 29.7 & 33.5 && 16.2 & 19.5 && 30.3 & 35.9 && 39.9 & 46.7 && 10.8 & 14.8 && 17.0 & 21.6 && 24.1 & 29.1 && 21.7 & 27.3 \\
\textsc{XLMR+Sap}$_{\text{all\_syn}}$ & 78.2 & 81.0 && 56.4 & 62.7 & & 31.8 & 37.3 && 18.6 & 22.2 && 35.4 & 41.2 && 42.8 & 48.9 && 16.7 & 21.4 && 18.8 & 23.0 && 24.0 & 28.1 && 20.6 & 27.5   \\
\hline  
%\small\color{red} Latest results (general-domain parallel data):\\
%  \textsc{XLMR+Sap}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de wt}}$ \textsc{XLMR} & & & &&&  & 13.2 & 18.1\\
%   \textsc{XLMR+Sap}$_{\text{en\_syn}}$$\xleftarrow{\text{en-de muse}}$ \textsc{XLMR} & & & & &&&  6.8 & 9.8 \\
%  %\textsc{XLMR+SapBert}$_{\text{en\_syn}}$$\xleftarrow{\text{en-zh wt}}$ \textsc{XLMR} \\
% \textsc{XLMR+Sap}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th wt}}$ \textsc{XLMR} & &  & && && & &&& & && && && && && &&&  &&&  1.4 & 3.7 \\
% \textsc{XLMR+Sap}$_{\text{en\_syn}}$$\xleftarrow{\text{en-th muse}}$ \textsc{XLMR} & & &&&  &&&   & && && && && && && && &&  &&& 0.1 & 0.2 \\
 \textsc{XLMR+Sap}$_{\text{en\_syn}}$(+en-lang wt) & -& - && 55.0 & 62.2 & & 34.6 & 41.4 && 18.6 & 24.4 && 35.0 & 41.5 && 43.3 & 50.6 && 15.9 & 22.3 && 15.9 & 23.0 && 18.7 & 24.4 && 25.1 & 32.4 \\
 \textsc{XLMR+Sap}$_{\text{en\_syn}}$(+en-lang muse) & - &-&&  54.4 & 61.0 && 28.7 & 34.4 && 16.7 & 20.6 && 33.6 & 39.0 && 41.9 & 48.8 && 11.9 & 16.3 && 12.3 & 16.7 && 15.7 & 19.9 && 18.6 & 25.1 \\
 \textsc{XLMR+Sap}$_{\text{en\_syn}}$(+en-lang wt+muse) & - & - && 49.4 & 59.6 &  & 30.3 & 36.9 && 20.4 & 28.9 && 33.2 & 41.9 && 42.7 & 51.7 &&  16.1 & 22.3 && 16.0 & 22.9 && 17.8 & 24.3 && 26.2 & 34.0  \\
%  \hdashline
%  \textsc{XLMR+Sap}$_{\text{en-tgt\_syn}}$(+en-lang wt) & - & - &&  & \\
%  \textsc{XLMR+Sap}$_{\text{en-tgt\_syn}}$(+en-lang muse) & - & - &&  \\
%  \textsc{XLMR+Sap}$_{\text{en-tgt\_syn}}$(+en-lang wt+muse) & - &- && \\
 \hdashline
  \textsc{XLMR+Sap}$_{\text{all\_syn}}$(+en-lang wt) & - & - && 57.2 & 63.7  && 35.1 & 42.3 && 20.3 & 27.6 && 35.8 & 43.8 && 48.8 & 55.0 && 22.1 & 27.9 && 20.6 & 27.3 && 24.8 & \textbf{31.3} && 30.0 & 37.6 \\
    \textsc{XLMR+Sap}$_{\text{all\_syn}}$(+en-lang muse) & - & - &&  57.9 & 63.9 && 33.0 & 38.4 && 23.0 & 27.3 && 39.8 & 45.9 && 47.2 & 54.5 && 22.1 & 25.7 && 19.2 & 25.6 && \textbf{25.2} & 30.2 && 25.9 & 32.8  \\
  \textsc{XLMR+Sap}$_{\text{all\_syn}}$(+en-lang muse+wt) & - & - &&  51.4 & 61.2 && 31.3 & 38.9 && 22.8 & 28.4 && 36.4 & 45.2 && 42.2 & 51.6 && \textbf{24.4} & \textbf{29.2} && 21.1 & 28.2 && 23.2 & 30.4 && \textbf{30.9} & \textbf{37.9} \\
\hdashline
  \textsc{mBert+Sap}$_{\text{all\_syn}}$(+en-lang wt) & - & - && 59.2 & 66.9 && \textbf{37.5} & \textbf{43.9} && 25.6 & 33.0 && 39.6 & 47.2 && 52.7 & 59.7 && 19.8 & 24.3 && 24.1 & 31.9 && 23.5 & 28.7 && 4.8 & 5.9 \\
  \textsc{mBert+Sap}$_{\text{all\_syn}}$(+en-lang muse) & - & - && 59.9 & 66.2 && 34.3 & 38.8 && 21.6 & 27.5 && 36.5 & 41.7 && 51.0 & 56.7 && 18.1 & 21.2 && 22.2 & 26.4 && 22.0 & 25.5 && 3.4 & 3.8\\
  \textsc{mBert+Sap}$_{\text{all\_syn}}$(+en-lang muse+wt) & - & - && 59.2 & \textbf{67.5} && 35.3 & 42.4 && \textbf{30.5} & \textbf{37.3} && \textbf{41.6} & \textbf{49.2} && \textbf{57.2} & \textbf{64.7} && 19.8 & 25.0 && \textbf{24.6} & \textbf{32.1} && 24.3 & 28.0 && 5.2 & 6.3 \\
\bottomrule
\end{tabular}
\caption{Zero-shot results on 1k randomly selected test set. All mentions in the 1k set have different surface forms from their linked titles. Note that for speeding up testing, the target ontology is a subset of UMLS: only the concepts appear in WikiMed are included. Without explicit mentioning, \texttt{[CLS]} is used as the representation. \textbf{Notations}: ``\textsc{Sap}'' means applying the \textsc{SapBert} pretraining method by \citet{liu2020self}; ``lang/\textsc{lang}'' means language of the column; ``tgt'' includes all tested languages that are in UMLS (i.e. es, de, fi, ru, tr, ko, zh);``$\leftarrow$'' means knowledge distillation \citep{reimers2020making}; ``(+$\cdot$)'' means further pre-training;``wt'' means Wikipedia title pairs (collected from latest wiki dump); ``muse'' means word translation pairs (\url{https://github.com/facebookresearch/MUSE}).}
%\vspace{-1.5em}
\end{table*}


